Private and Atomic Exchange of Assets over Zero Knowledge Based Payment Ledger

Bitcoin brings a new type of digital currency that does not rely on a central system to maintain transactions. By benefiting from the concept of decentralized ledger, users who do not know or trust each other can still conduct transactions in a peer-to-peer manner. Inspired by Bitcoin, other cryptocurrencies were invented in recent years such as Ethereum, Dash, Zcash, Monero, Grin, etc. Some of these focus on enhancing privacy for instance crypto note or systems that apply the similar concept of encrypted notes used for transactions to enhance privacy (e.g., Zcash, Monero). However, there are few mechanisms to support the exchange of privacy-enhanced notes or assets on the chain, and at the same time preserving the privacy of the exchange operations. Existing approaches for fair exchanges of assets with privacy mostly rely on off-chain/side-chain, escrow or centralized services. Thus, we propose a solution that supports oblivious and privacy-protected fair exchange of crypto notes or privacy enhanced crypto assets. The technology is demonstrated by extending zero-knowledge based crypto notes. To address "privacy" and "multi-currency", we build a new zero-knowledge proving system and extend note format with new property to represent various types of tokenized assets or cryptocurrencies. By extending the payment protocol, exchange operations are realized through privacy enhanced transactions (e.g., shielded transactions). Based on the possible scenarios during the exchange operation, we add new constraints and conditions to the zero-knowledge proving system used for validating transactions publicly.

==> sec-background.tex <==

% crypto tools go here
\section{Background}
\label{sec-background}

%\subsection{Background of Zero-knowledge}
A zero-knowledge proof of knowledge is a protocol in which a prover can convince a verifier that some statement holds without revealing any information.

Roughly speaking, a zero-knowledge proof involves two parties, the {\it prover} and the {\it verifier}. For a statement, the {\it prover} can generate a proof to convince the {\it verifier} of the correctness of the statement. In this process, the {\it verifier} cannot learn anything except the fact that the statement is true (zero-knowledge feature). Zero-knowledge proofs can be either interactive or non-interactive.
Interactive zero-knowledge proofs ~\cite{goldwasser1985knowledge,goldreich1996construct} requires the {\it prover} to communicate with the {\it verifier} over multiple rounds to finish the proof.
Non-interactive zero-knowledge proofs (NIZK)~\cite{blum1988non,groth2006perfect,de2001robust} do not require multiple rounds of interactions between {\it prover} and {\it verifier} and are more suitable for scenarios where it is hard for these parties to be online at the same time.

An important tool related to NIZK is zero-knowledge succinct non-interactive arguments of knowledge (zk-SNARK)~\cite{gennaro2013quadratic,ben2013snarks,ben2014succinct}. zk-SNARK allows for efficient verification of NP statements with proofs produced by an untrusted but computationally bounded prover. A trusted party is used to publish a proving key and verification key, where the proving key is used to generate non-interactive proofs for adaptively-chosen NP statements, and the verification key is used to verify the proof.
We refer the readers to~\cite{ben2013snarks} for a more formal definition of zk-SNARK.

%\input{subsec-preliminaries}



\iffalse
There are several implementations/libraries available in the community, e.g. Pinocchio~\cite{parno2013pinocchio} and zk-SNARKs. As zk-SNARKs has already been used in many privacy-concerned blockchain systems like Zcash, in this paper, we utilize zk-snark as an example, to explain how we implement our privacy-preserving exchange system protocol.

A significant concept of zk-snark is \textit{Homomorphic Hiding (HH)}. An \textit{HH} function $E(x)$ can be described as follows~\cite{zcash2018hh}.
\begin{enumerate}
    \item It is difficult to revert recovery $x$ even if the value of $E(x)$ is known;
    \item If $x$ is not equal to $y$, then $E(x)$ is not equal to $E(y)$;
    \item If both $E(x)$ and $E(y)$ are known, then the value of HH of arithmetic expressions can also be calculated, e.g., $E(x+y)$.
\end{enumerate}
Then we can use \textit{HH} to evaluate a polynomial "blindly". That is to say, suppose that we have two subjects Alice and Bob, and Alice knows a $d$-degree polynomial:
$$
\begin{aligned}
    P(X)=a_0+a_1X+a_2X^2+...+a_dX^d
\end{aligned}
$$
And, Bob wants to know the value of $E(P(s))$ which is relevant to $s$. During the evaluation, Alice only knows $P$ and does not know $s$ and meanwhile, Bob only knows $s$ and does not know $P$. 

So far we may be starting to see some signs of zero-knowledge proof with \textit{Homomorphic Hiding} and \textit{Blind Evaluation of Polynomial}. The next step is to convert our statements or constraints in the knowledge into polynomials. For example, if Alice wants to prove that she knows a value $x$ which satisfy the evaluation:
$$
\begin{aligned}
    x^2+2x+1=out
\end{aligned}
$$
Note that $out$ is a public knowledge here. By introducing some intermediate variables, this equations can be further decomposed into several basic arithmetic expressions:
$$
\begin{aligned}
    &x*x=var_1\\
    &2*x=var_2\\
    &var_1+var_2=var_3\\
    &var_3+1=out
\end{aligned}
$$
More formally, it can be converted to R1CS, i.e. for a vector $(a,b,s)$, we always have $s=a*b$.
$$
\begin{aligned}
    &var_1=x*x\\
    &var_2=2*x\\
    &var_3=(var_1+var_2)*1\\
    &out=(var_3+1)*1
\end{aligned}
$$
With R1CSs, we can start to translate them into one about polynomials using QAPs. In the following section, we will discuss this procedure in details. In summary, now we have initialized a zero-knowledge proof system. We may still need some other techniques like \textit{Pinocchio} and \textit{Elliptic Curves}~\cite{miller1985use} to complete the whole system, but they are out of the scope of this paper.
\fi

==> sec-case-study.tex <==

\section{Case Study}

\subsection{Common Cases}
%\subsection{An example of privacy swap}

\begin{table}
\centering
\caption{Spending cases based note type $<T^{old},T^{new}>$}
\label{table-cases}
\begin{tabularx}{0.9\columnwidth}{|l|l|l|X|} 
\hline
Input                       & Debt? & Output    & Cases     \\ 
\hline
$<0,0>$                     & No    & $<0,0>$   & Case 1    \\ 
\cline{3-4}
                             &       & $<0,1>$  & Case 4    \\ 
\cline{3-4}
                             &       & $<1,1>$  & X         \\ 
\cline{2-4}
                            & YES    & $<0,0>$  & Case 3    \\ 
\cline{3-4}
                             &       & $<0,1>$  & Case 3 $\rightarrow$ Case 4           \\ 
\cline{3-4}
                             &       & $<1,1>$ & X          \\ 
\hline
$<0,1>$ & NO    & $<0,0>$ & Case 5: Subcase 1               \\ 
\cline{3-4}
                             &       & $<0,1>$ & Case 5: Subcase 2                                \\ 
\cline{3-4}
                             &       & $<1,1>$ & X          \\ 
\cline{2-4}
                             & YES   & $<0,0>$ & Case 2: Subcase 1 or Case 6  \\ 
\cline{3-4}
                             &       & $<0,1>$ & Case 2: Subcase 2                              \\ 
\cline{3-4}
                             &       & $<1,1>$ & X        \\ 
\hline
$<1,1>$ & NO    &                              & X       \\ 
\cline{2-4}
                             & YES   &                              & X                         \\
\hline
\end{tabularx}
\end{table}

\para{Assumptions.}
\begin{inparaenum}[1)]
    \item For every transaction, we restrict to 2 input and 2 output notes; and
    \item Input or output note can be dummy note (no commitment); and
    \item Spending cases of more than 2 input notes or 2 output notes can be reduced to transactions with 2 notes; and
    \item Use Zcash as reference model and zk-snark tool (notations based on Zcash); and
    \item Extend to other zk schemes or tools (common string without secure setup or not based on tinyRAM model~\cite{ben2013snarks}).
\end{inparaenum}

\figurename~\ref{fig-ideal-case} shows an ideal case for this atomic swap operation. As it defines $\mathit{T}$, $\mathit{C}$, $\mathit{V}$ in Section~\ref{sec-formal-definition}, we have: 

\begin{figure}
    \centering
    \includegraphics[width=3in]{fig-ideal-case}
    \caption{Ideal swap scenario}
    \label{fig-ideal-case}
\end{figure}

\para{Case 1: Non-swap-related transactions.}

Matching conditions:
\begin{subequations}
$$ \left\{
\begin{aligned}
&T^{old}_1  =  T^{old}_2 =  T^{new}_1 = T^{new}_2 =0 \\
&V^{old}_{1,2}  =  V^{old}_{2,2} =  V^{new}_{1,2} = V^{new}_{2,2} =0 \\
&C^{old}_1  =  C^{old}_2 =  C^{new}_1 = C^{new}_2 \\
&V^{old}_{pub,color} + \sum_{i=1}^{N^{old}} V^{old}_{i,1} = V^{new}_{pub,color} + \sum_{i=1}^{N^{new}} V^{new}_{i,1}
\end{aligned}
\right.
$$
\end{subequations}

Suppose a note can be denoted simply as $[T,C_1,V_1,C_2,V_2]$, and are splitting 5 units for green note (color code: 3) into 3 and 2 units, we have 
\iffalse
\begin{subequations}
$$ \left \{ 
\begin{aligned}
[0,(3,5),(0,0)] \\
[0,(0,0),(0,0)]
\end{aligned}
\right \} \rightarrow \left \{ 
\begin{aligned}
[0,(3,3),(0,0)] \\
[0,(3,2),(0,0)]
\end{aligned}
\right \}
$$
\end{subequations}
\fi

\begin{figure}[h]
    \centering
    \includegraphics[width=4.2in]{fig-case-1}
    \caption{Case 1 example.}
    \label{fig-case-1}
\end{figure}

Note that if $C=0$, we consider it as a dummy note (e.g. input note 2 in \figurename~\ref{fig-case-1}). It is used only when splitting one note into two. 

\para{Case 2: Swap setup.} Alice initiates the swap.

Matching conditions:
\begin{subequations}
$$ \left\{
\begin{aligned}
&T^{old}_1 =T^{old}_2 = 0 \\
&(V^{old}_{1,2}  = V^{old}_{2,2}  = 0 &or \\
&V^{old}_{1,2} >0,V^{old}_{2,2} = 0 &or\\
&V^{old}_{1,2} =0,V^{old}_{2,2} > 0) \\
&T^{new}_1  =T^{new}_2 = 1 \\
&V^{new}_{1,2}  > 0 \\
&V^{new}_{2,2}  = 0 \\
\end{aligned}
\right.
$$
\end{subequations}

Suppose a note can be denoted simply as $[T,C_1,V_1,C_2,V_2]$, and Alice creates 5 units of green note to exchange 7 units of red note (color code: 2) from Bob, we have 
\iffalse
\begin{subequations}
$$ \left \{ 
\begin{aligned}
[0,(3,5),(0,0)] \\
[0,(0,0),(0,0)]
\end{aligned}
\right \} \rightarrow \left \{ 
\begin{aligned}
[0,(3,5),(2,7)] \\
[1,(2,7),(0,0)]
\end{aligned}
\right \}
$$
\end{subequations}
\fi

\begin{figure}[h]
    \centering
    \includegraphics[width=2in]{fig-case-2}
    \caption{Case 2 example.}
    \label{fig-case-2}
\end{figure}

Note that output note (sibling note) $[1,2,7,0,0]$ cannot be spent unless output note $[0,3,5,2,7]$ is spent. $[0,3,5,2,7]$ has a negative part where $C_2=2$ and $V_2=7$.

Additional verification for this case, besides the original verification for privacy-based cryptocurrency like ZCash~\cite{hopwood2016zcash}:

When $V^{old}_{1,2}  = V^{old}_{2,2}  = 0$, we verify
\begin{subequations}
$$ \left\{
\begin{aligned}
&C^{old}_{1,1}=C^{old}_{2,1}=C^{new}_{1,1} \\
&C^{new}_{1,2}=C^{new}_{2,1} \\
&V^{new}_{1,2}=V^{new}_{2,1} \\
&V^{old}_{1,1} + V^{old}_{2,1}=V^{new}_{1,1}
\end{aligned}
\right.
$$
\end{subequations}

When $V^{old}_{1,2}  > 0$, we verify

When $V^{old}_{2,2}  > 0$, we verify

\para{Case 3: Swap cancellation.} Alice cancels the swap. In another word, Alice spends before Bob and gets the notes back.

Matching conditions:
\begin{subequations}
$$ \left\{
\begin{aligned}
&T^{old}_1  = 0 \\
&T^{old}_2 = 1 \\
&V^{old}_{1,2}  > 0 \\
&V^{old}_{2,2} = 0 \\
&(T^{new}_1=0, T^{new}_2=0, V^{new}_{1,2}=0, V^{new}_{2,2}=0 &or\\
&T^{new}_1=0, T^{new}_2=1, V^{new}_{1,2}>0, V^{new}_{2,2}=0)
\end{aligned}
\right.
$$
\end{subequations}

Suppose a note can be denoted simply as $[T,C_1,V_1,C_2,V_2]$, and we recover 5 units of green note and 7 units of requested red note back to previous status, we have 

\iffalse
\begin{subequations}
$$ \left \{ 
\begin{aligned}
[0,(3,5),(2,7)] \\
[1,(2,7),(0,0)]
\end{aligned}
\right \} \rightarrow \left \{ 
\begin{aligned}
[0,(3,3),(0,0)] \\
[0,(3,2),(0,0)]
\end{aligned}
\right \}
$$
\end{subequations}
\fi

\begin{figure}[h]
    \centering
    \includegraphics[width=2in]{fig-case-3}
    \caption{Case 3 example.}
    \label{fig-case-3}
\end{figure}

Additional verification for this case:

When $V^{new}_{1,2}  = V^{new}_{2,2}  = 0$, we verify
\begin{subequations}
$$ \left\{
\begin{aligned}
&C^{old}_{1,2}=C^{old}_{2,1}\\
&C^{new}_{1,1}=C^{new}_{2,1}=C^{old}_{1,1} \\
&V^{new}_{1,2}=V^{new}_{2,1} \\
&V^{new}_{1,1} + V^{new}_{2,1}=V^{old}_{1,1}
\end{aligned}
\right.
$$
\end{subequations}

When $T^{new}_2=1$ and $V^{new}_{1,2}>0$: ...

\para{Case 4: Swap beginning.} In order to spend the note, Bob needs to handle the note with negative value.

Matching conditions:
\begin{subequations}
$$ \left\{
\begin{aligned}
&T^{old}_1 = T^{old}_2 = T^{new}_1 = T^{new}_2 = 0 \\
&(V^{old}_{1,2}>0, V^{old}_{2,2}=0 & or \\
&V^{old}_{1,2}=0, V^{old}_{2,2}>0) \\
&V^{new}_{1,2}=0, V^{new}_{2,2}=0
\end{aligned}
\right.
$$
\end{subequations}

Suppose a note can be denoted simply as $[T,C_1,V_1,C_2,V_2]$, and Bob receives 5 units of green note by sending 9 units of red note to cancel the negative value, we have 
\iffalse
\begin{subequations}
$$ \left \{ 
\begin{aligned}
[&0,(3,5),(2,7)] \\
[&0,(2,10),(0,0)]
\end{aligned}
\right \} \rightarrow \left \{ 
\begin{aligned}
[0,(3,5),(0,0)] \\
[0,(2,3),(0,0)]
\end{aligned}
\right \}
$$
\end{subequations}
\fi

\begin{figure}[h]
    \centering
    \includegraphics[width=2in]{fig-case-4}
    \caption{Case 4 example.}
    \label{fig-case-4}
\end{figure}

When $V^{old}_{1,2}>0$ and $C^{old}_{1,1}=C^{new}_{1,1}$, we verify
\begin{subequations}
$$ \left\{
\begin{aligned}
&V^{old}_{1,1}=V^{new}_{1,1} \\
&C^{old}_{1,2}=C^{old}_{2,1}\\
&C^{old}_{2,1}=C^{new}_{2,1} \\
&V^{old}_{1,2} + V^{new}_{2,1}=V^{old}_{2,1} \\
&block_n \geq bt^{old}_1
\end{aligned}
\right.
$$
\end{subequations}

When $V^{old}_{1,2}>0$ and $C^{old}_{1,1}=C^{new}_{2,1}$: ...

When $V^{old}_{2,2}>0$ and $C^{old}_{2,1}=C^{new}_{1,1}$: ...

When $V^{old}_{2,2}>0$ and $C^{old}_{2,1}=C^{new}_{2,1}$: ...

\para{Case 5: Swap completion.} Alice spends after Bob.

Matching conditions:
\begin{subequations}
$$ \left\{
\begin{aligned}
&T^{old}_1 = 1 \\
&T^{old}_2 = 0 \\
&V^{old}_{1,2} = V^{old}_{2,2} = 0 \\
&(T^{new}_1 = 0, T^{new}_2 = 0, V^{new}_{1,2}=0, V^{new}_{2,2}=0 & or \\
&T^{new}_1 = 0, T^{new}_2 = 1, V^{new}_{1,2}>0, V^{new}_{2,2}=0) \\
\end{aligned}
\right.
$$
\end{subequations}

Suppose a note can be denoted simply as $[T,C_1,V_1,C_2,V_2]$, and Alice spends the red note, we have 

\iffalse
\begin{subequations}
$$ \left \{ 
\begin{aligned}
[1,(2,7),(0,0)] \\
[0,(0,0),(0,0)]
\end{aligned}
\right \} \rightarrow \left \{ 
\begin{aligned}
[0,(2,4),(0,0)] \\
[0,(2,3),(0,0)]
\end{aligned}
\right \}
$$
\end{subequations}
\fi

\begin{figure}[h]
    \centering
    \includegraphics[width=2in]{fig-case-5}
    \caption{Case 5 example.}
    \label{fig-case-5}
\end{figure}

Note that input note 1 can only be spent if there is a matching nullifier for a note already spent by Bob that matches with input note 1 (See Case 4).

Additional verification for this case:
When $T^{new}_1=T^{new}_2=V^{new}_{1,2}=0$, we verify
\begin{subequations}
$$ \left\{
\begin{aligned}
&C^{old}_{1,2}=C^{old}_{2,1}=C^{new}_{1,2}=C^{new}_{2,1}\\
&V^{old}_{1,2} + V^{old}_{2,1}=V^{new}_{1,2}+V^{new}_{2,1} \\
&block_n > bt^{old}_1\\
&T^{old}_1=1\\
&\exists n^{old}_3 \wedge h^{old}_{3,sig}= h^{old}_{1,sig}\\
&(\exists cm^{old}_3\ with\ Merkle\ path\ (path3, pos3)\ respect\ to\\ 
&rt \wedge cm^{old}_3 = NoteCommit(n^{old}_3))\\
&(\exists nf^{old}_3\ with\ Merkle\ path\ (path4,pos4)\ respect\ to\\
&rt \wedge nf^{old}_3 = PRF^{nf}_{a^{old}_{sk,3}}(\rho^{old}_3))\\
&|pos3 = pos1| <2
\end{aligned}
\right.
$$
\end{subequations}

Additional subcases:
When $T^{new}_2=1$ and $V^{new}_{1,2}>0$:
...

\para{Case 6: Swap completion (Another case).} Alice spends before Bob.

Matching conditions:
\begin{subequations}
$$ \left\{
\begin{aligned}
&T^{old}_1 = 1 \\
&T^{old}_2 = 0 \\
&V^{old}_{1,2} >0\\
&V^{old}_{2,2} = 0 \\
&T^{new}_1 = 0, T^{new}_2 = 0, V^{new}_{1,2}=0, V^{new}_{2,2}=0\\
\end{aligned}
\right.
$$
\end{subequations}

Suppose a note can be denoted simply as $[T,C_1,V_1,C_2,V_2]$, we have 
\iffalse
\begin{subequations}
$$ \left \{ 
\begin{aligned}
[1,(2,7),(0,0)] \\
[0,(3,1),(2,5)]
\end{aligned}
\right \} \rightarrow \left \{ 
\begin{aligned}
[0,(2,2),(0,0)] \\
[0,(3,1),(0,0)]
\end{aligned}
\right \}
$$
\end{subequations}
\fi

\begin{figure}[h]
    \centering
    \includegraphics[width=2in]{fig-case-6}
    \caption{Case 6 example.}
    \label{fig-case-6}
\end{figure}

Additional verification for this case:
When $T^{new}_1=T^{new}_2=V^{new}_{1,2}=0$, we verify
\begin{subequations}
$$ \left\{
\begin{aligned}
&C^{old}_{1,1}=C^{old}_{2,2}=C^{new}_{1,1}\\
&C^{old}_{2,1}=C^{new}_{2,1} \\
&V^{old}_{1,1} = V^{old}_{2,2}+V^{new}_{1,1} \\
&V^{old}_{2,1} = V^{new}_{2,1} \\
&block_n > bt^{old}_1\\
&block_n \leq bt^{old}_2\\
&\exists n^{old}_3 \wedge h^{old}_{3,sig}= h^{old}_{1,sig}\\
&(\exists cm^{old}_3\ with\ Merkle\ path\ (path3, pos3)\ respect\ to\\ 
&rt \wedge cm^{old}_3 = NoteCommit(n^{old}_3))\\
&(\exists nf^{old}_3\ with\ Merkle\ path\ (path4,pos4)\ respect\ to\\
&rt \wedge nf^{old}_3 = PRF^{nf}_{a^{old}_{sk,3}}(\rho^{old}_3))\\
&|pos3 = pos1| <2
\end{aligned}
\right.
$$
\end{subequations}

\para{Other cases.} Reject because all valid spending scenarios can be decomposed using case 1-6.

\subsection{Circuit Design}
As we discussed in the previous sections, zero-knowledge allows anyone to verify a transaction without complete information from a prover. It means that the system does not need to provide information (e.g. amounts, coin types etc.) but the verifier can still evaluate the preset conditions. There are several tools and libraries available to achieve this goal. For example, Pinocchio~\cite{parno2013pinocchio}, zk-snark~\cite{sasson2014zerocash}, and Geppetto~\cite{costello2015geppetto}. In common, zero-knowledge requires a complex circuit to generate proofs and keys for the verifiers. Graig \emph{et al.} propose an approach to reduce the complexity of the circuit, save energy and increase the performance. \figurename~\ref{fig-simple-circuit} illustrates a customized design for our cases. Suppose that each sub circuit in the figure handle one spending case. The original design (left) requires the system to execute all circuit and uses a multiplexer to select the output. Instead, an optimized scheme is to select a sub circuit by a multiplexer before execution (right). The control signal of the multiplexer is from the \textit{Matching Conditions} of every case. \tablename~\ref{table-cases} also describes those conditions in high level. As a result, the system does not need to handle other non-selected circuits.

\begin{figure}
    \centering
    \includegraphics[width=3in]{fig-simple-circuit}
    \caption{An optimal circuit design}
    \label{fig-simple-circuit}
\end{figure}

In this section, we will use a zk-snark library \textit{libsnark} to build the prototype of the proving system~\cite{ben2013snarks}. Similar to electrical engineering, circuits should be attached to a protoboard in order to connect every component in the circuit. The major elements in the virtual circuit of zk-snark are R1CS. An R1CS is a vector of $(a, b, s)$, where $s=a*b$. As a result, each R1CS can be considered as an arithmetic gate of multiplication (See \figurename~\ref{fig-r1cs}). 

\begin{figure}[h]
    \centering
    \includegraphics[width=1in]{fig-r1cs}
    \caption{Many R1CS gates integrate and form a circuit.}
    \label{fig-r1cs}
\end{figure}

An arithmetic expression can be further decomposed in a set of R1CS. For instance, if the system needs to verify $V^{old}_{1,1} + V^{old}_{2,1}=V^{new}_{1,1}$, it can be transformed into an R1CS expression $(V^{old}_{1,1} + V^{old}_{2,1} - V^{new}_{1,1})*1=0$, where $a=(V^{old}_{1,1} + V^{old}_{2,1} - V^{new}_{1,1})$, $b=1$ and $s=0$. For boolean expression, we can restrict the value to $0$ or $1$, e.g. $s*(1-s)=0$ means $s$ can be only $0$ or $1$.

In \textit{libsnark}, we implement a R1CS constraint as following:

\lstset{language=C++,
                basicstyle=\ttfamily,
                keywordstyle=\color{blue}\ttfamily,
                stringstyle=\color{red}\ttfamily,
                commentstyle=\color{green}\ttfamily,
                morecomment=[l][\color{magenta}]{\#}}
\begin{lstlisting}
    //pb is the protoboard.
    this->pb.add_r1cs_constraint(
        r1cs_constraint<FieldT>(a,b,s));
\end{lstlisting}

And, generate a proof for the circuit:
\begin{lstlisting}
    //s=a*b
    this->pb.val(s) = 
        this->pb.val(a) * this->pb.val(b);
\end{lstlisting}

Note that we also need to generate a key pair of $<proof-key,verify-key>$ to use in a zk-proof system. Eventually, a verifier just needs the $verify-key$, public inputs, and the proof to verify a transaction.


==> sec-exp.tex <==
\section{Implementation and Experiments}\label{sec-exp}
This section presents the implementation of the proposed exchange scheme and evaluates its performance.

\input{subsec-circuit-design}
\input{subsec-circuit-evaluation} 

==> sec-security-model.tex <==
\section{Security Model}\label{sec-formal-definition}

Intuitively, a privacy-preserving decentralized swap (PDS) scheme on decentralized ledger should satisfy three features:
\begin{inparaenum}[(i)]
    \item Fairness. When two users agree to do an exchange of crypto assets, the operation leads to two possibilities: it fails that each one still has his/her note, or it succeeds that each one possesses the other's note (type and amount).
    \item Privacy. Though all transaction information is stored on the decentralized ledger, other users should not be able to learn any useful information about the swap transaction.
    \item Verifiability. The public should be able to verify the validity of all transactions and prevent double spending.
\end{inparaenum}

A privacy-preserving asset swap scheme on decentralized ledger should further satisfy the following requirements.

\begin{defn}[Transaction Indistinguishability]\label{def-ind-tx}
    Given the blockchain with many transactions, the challenger $\mathcal{C}$ selects two transactions, one is created by $\mathcal{C}$ and the other is created by others.
    $\mathcal{C}$ is then randomly selects a bit $b$, and sets $\textit{tx}_b$ the transaction of $\mathcal{C}$. The other transaction is denoted as $\textit{tx}_{1-b}$.
    The adversary $\mathcal{A}$ is given information of $\mathcal{C}$, and two transactions $\textit{tx}_0$ and $\textit{tx}_1$. The adversary then tries to find out $b'$ such that $b=b'$. If the success probability is negligible, the ExDL scheme is transaction indistinguishable. 
\end{defn}


\iffalse
Before giving the formal definitions that capture the intuition, we first describe the formal definition of a decentralized ledger based swap scheme.

\subsection{Data Structures of PDS}
A PDS scheme is built on several data structures and summarize these structures here.
\begin{itemize}
    \item Ledger.
    \item 
\end{itemize}

\begin{defn}[Privacy preserving decentralized asset swap]\label{def-exchange}
An asset swap scheme on decentralized ledger consists of four algorithms:
\begin{itemize}
    \item \texttt{Setup}. This function takes as input the security parameter and other configurations, and outputs all public parameters and sets up the system.
    \item \texttt{TxInitialize}. This function takes as input two crypto assets of different types and creates a transaction to initialize a swap.
    \item \texttt{TxClose}. This function takes as input a transaction of swap initialization and creates a transaction to close the swap. The close transaction may lead to one of two results: the swap succeeds and each party gets the other's asset, or the swap fails and each party gets back his/her own asset.
    \item \texttt{TxVerify}. This function takes as input a transaction (either swap initialization or swap close), and the current version of the decentralized ledger, and outputs \textit{valid} or \textit{invalid}.
\end{itemize}
\end{defn}

Besides these four essential functions, other supporting functions are common for all decentralized ledgers, such as block construction, consensus, and branch selection.

An ExDL $\mathcal{E}$ should satisfy the following basic requirements.

\begin{defn}[Public verifiability]\label{def-public-verifiablity}
    Given the current blockchain and a new transaction, everyone can verify whether the transaction is valid or not.
\end{defn}

\begin{defn}[Atomic]\label{def-atomic}
    \texttt{TxInitialize} and \texttt{TxClose} are atomic, i.e., the execution of a function either succeeds or fails, but it will not terminate in the middle.
\end{defn}

\begin{defn}[Completeness]\label{def-completeness}
    \texttt{TxInitialize} and \texttt{TxClose} always appears in pair for involved assets.
    For an asset, there is one and only one pair of \texttt{TxInitialize} and \texttt{TxClose} transactions in the system at one time. 
\end{defn}
\fi



==> subsec-circuit-design.tex <==
\subsection{Arithmetic Circuit Design for OMAP}

As discussed in the previous sections, zero-knowledge proving system allows anyone to verify a transaction without complete information from a prover. It means that the system does not need to provide private transaction information (e.g., amounts, asset types, etc.). The verifier can still validate if the transaction instance satisfies the preset conditions. There are several tools and libraries available to achieve this goal. For example, Pinocchio~\cite{parno2013pinocchio}, zk-SNARK~\cite{sasson2014zerocash}, and Geppetto~\cite{costello2015geppetto}. In common, zero-knowledge proving system requires a complex circuit to generate proofs and verifying keys for the verifiers. Graig \emph{et al.} propose an approach to reduce the complexity of the circuit, save energy and increase the performance. \figurename~\ref{fig-simple-circuit} illustrates a customized design for our extended JoinSplit transaction cases. Suppose that each sub-circuit in the figure handles one JoinSplit spending case. Each sub-circuit checks the satisfiability of the transaction information. The results are combined together using logical operation. 

In the experiment implantation, we use a zk-SNARK library \textit{libsnark} to build the prototype of the proving system~\cite{ben2013snarks}. Circuits should be attached to a protoboard in order to connect every component in the circuit. The major elements in the virtual circuit of zk-SNARK are R1CS. An R1CS is a vector of $(a, b, s)$, where $s=a*b$. As a result, each R1CS can be considered as an arithmetic gate of multiplication. An arithmetic expression can be further decomposed in a set of R1CS. For instance, if the system needs to verify $v^{old}_{1,1} + v^{old}_{2,1}=v^{new}_{1,1}$, it can be transformed into an R1CS expression $(v^{old}_{1,1} + v^{old}_{2,1} - v^{new}_{1,1})*1=0$, where $a=(v^{old}_{1,1} + v^{old}_{2,1} - v^{new}_{1,1})$, $b=1$ and $s=0$. For Boolean expression, we restrict the value to $0$ or $1$, e.g. $s*(1-s)=0$ means $s$ can be only $0$ or $1$.

The existing code base developed for Zcash is used as the baseline. Necessary changes are made to implement and test the described OMAP system. A proving system is used to generate a proof for each JoinSplit transaction based on the extended data models and algorithms. Note that we need to generate a key pair of $<$\textit{pk},\textit{vk}$>$ to use in a ZK proving system. Eventually, a verifier just needs the \textit{vk}, public inputs $\chi$, and the proof $\pi$ to verify a transaction.

Since the proving system for JoinSplit transactions handles parallel spending cases, the proving circuit can be further optimized by dividing it into sub-circuits. The original design (left) requires the system to execute all circuit and uses a multiplexer to select the output. Instead, an optimized scheme is to select a sub-circuit by a multiplexer before execution (right). The control signal of the multiplexer is from the \textit{satisfying conditions} of every spending case. %\tablename~\ref{table-cases} also describes those conditions in high level. 
As a result, the system does not need to handle other non-selected circuits.
\begin{figure}
    \centering
    \includegraphics[width=3.6in]{fig-simple-circuit}
    \caption{An optimal circuit design.}
    \label{fig-simple-circuit}
\end{figure}


\iffalse
(See \figurename~\ref{fig-r1cs}). 
\begin{figure}[h]
    \centering
    \includegraphics[width=1in]{fig-r1cs}
    \caption{Many R1CS gates integrate and form a circuit.}
    \label{fig-r1cs}
\end{figure}
\fi
\iffalse
In \textit{libsnark}, we implement a R1CS constraint as following:

\lstset{language=C++,
                basicstyle=\ttfamily,
                keywordstyle=\color{blue}\ttfamily,
                stringstyle=\color{red}\ttfamily,
                commentstyle=\color{green}\ttfamily,
                morecomment=[l][\color{magenta}]{\#}}
\begin{lstlisting}
    //pb is the protoboard.
    this->pb.add_r1cs_constraint(
        r1cs_constraint<FieldT>(a,b,s));
\end{lstlisting}

And, generate a proof for the circuit:
\begin{lstlisting}
    //s=a*b
    this->pb.val(s) = 
        this->pb.val(a) * this->pb.val(b);
\end{lstlisting}
\fi




==> subsec-initialization.tex <==

\subsection{Note Initialization}
Before Alice can swap her asset $(t_1, v_1)$ with Bob in a privacy preserving way, she needs to initialize the swap by converting the asset to a new type of note. Alice does the following steps for the conversion:
\begin{enumerate}
    \item Serial number generation. Alice selects a random number $\rho_1$ as the serial number of the new note.
    \item Quid pro quo determination. Alice specifies the asset she wants to get from Bob, which is also identified as a pair $(t_2, v_2)$.
    \item Transaction construction. 
\end{enumerate}

==> subsec-preliminaries.tex <==

% high level idea goes here
\subsection{Preliminaries of Privacy Preserving Swap of Assets}\label{sec-overview}
In this section, we give preliminaries of the privacy swap mechanism on the decentralized ledger.

We assume there are more than one type of crypto assets in the system. The assets are private (e.g., privacy coins). Furthermore, owners of two different types of assets, Alice and Bob, want to exchange or swap the ownership on the multi-asset decentralized ledger that supports privacy swap of privacy protected assets. Here note is used to represent crypto asset. Privacy note means privacy enhanced note (e.g., Crypto note, Zcash). 
\subsubsection{Straightforward Approach}
If privacy is not a concern, we can implement swap as follows:
\begin{itemize}
    \item Alice and Bob achieve agreement to swap their notes off-chain.
    \item Alice initializes the swap operation by submitting a transaction to the blockchain, which includes information of the two notes, the identity of Alice and Bob, and their signatures of the transaction, which demonstrates that the two owners of the two notes agree to exchange.
    \item All nodes on the blockchain verify the transaction. If everything is ok, blockchain accepts the transaction and the swap is complete.
\end{itemize}
It is easy to see that this protocol can guarantee fairness of the exchange, i.e., at the end of the swap transaction, both Alice and Bob will get the other person's note.
However, this approach does not provide any privacy protection. Every node in the blockchain system can observe that there is a swap transaction between Alice and Bob. 
To protect Alice and Bob's privacy, we can leverage one-time wallet mechanism and ring signature for swap. The protocol works as follows:
\begin{itemize}
    \item Alice selects a one-time wallet and uses a ring signature based privacy preserving transfer mechanism to transfer her note to her one-time wallet.
    \item Bob does the same thing to transfer his note to his one-time wallet.
    \item The swap is carried out between the two one-time wallets as in the above exchange protocol without privacy protection.
\end{itemize}
Intuitively, this protocol provides better privacy protection because the public cannot link the swap transaction with Alice and Bob directly.
However, this approach also has its limitation, i.e., the actual exchange operation is still processed and stored on the ledger as plaintext. The public knows how many swaps that have happened and time of these swap transactions.  
The selection of ring members is also risky. If the members are not selected carefully, an adversary may collect useful information to reveal likely transaction embedded in the ring signature.
\subsubsection{Privacy Preserving Swap}
The proposed privacy preserving swap scheme leverages zero knowledge proof. It can be implemented as multi-asset and privacy swap extension to privacy coins such as Zcash. It works as follows:
\begin{itemize}
    \item Alice and Bob communicate off-chain and agree to swap their assets with each other. Without loss of generality, we suppose that Alice will initialize the swap operation.
    \item Alice first converts her asset into two notes (one for herself and one for Bob). The note for Bob includes two parts: one part stands for her asset with a positive value (both asset type and amount), one part stands for Bob's asset with a negative value (asset type and amount). The note for herself, paired with the previous note, has a positive value (asset type and amount) to cancel the negative part that is embedded in the previous note. Alice also creates a spending key that one can use to spend her newly created notes. All blockchain nodes verify the new notes and store them on the blockchain. When the two notes are spent together, Alice reclaims her asset back (denote the scenario that the swap operation is cancelled). 
    \item Alice and Bob exchange the spending secret so they can spend the shared note.
    \item If Bob spends Alice's note, he needs to spend his asset note to cancel the negative value of the note that he receives from Alice (both type and amount have to match).
\item After Bob spends the shared note, Alice can spend the second note that is created in pair with the note that is spent by Bob. To do so, Alice needs to show that the pairing note has been spent already by Bob in such a manner that it doesn’t disclose that there is a swap transaction. Similar to commitment pool of committed notes, there is a pool of nullifiers (notes spent already). Using zero knowledge proof, Alice can prove to others that her transaction is valid without disclosing that she is spending a note that links to a swap transaction with Bob. 
\end{itemize} 
In reality, the situation is more complicated as one party in the swap operation may cheat, which should be handled by the protocol.


==> subsec-primitive-tools.tex <==

\subsection{Primitive Tools of Privacy Swap on Blockchain}

==> subsec-terms.tex <==

\subsection{Terminology and Symbols}
Note that here we only list those symbols which are used in this paper. Refer to ~\cite{hopwood2016zcash} for a complete description of notations in the zero-knowledge proof system. The description is based on extending Zcash note format and operations. Here we skip definitions that can be found in the original Zcash publication and implementation specification.


\subsubsection{Public input}

Public input is the knowledge that is revealed to every participant in a transaction.
\begin{align*}
    \chi=&(rt,\mathit{nf}^{old}_1, \mathit{nf}^{old}_2, cm^{new}_1, cm^{new}_2, V^{old}_{pub,\mathit{color}}, V^{new}_{pub,color},\\
    &block_n,h_{sig},h_1,h_2) \\
    &\text{where} \\
    &rt: \text{merkle tree root.} \\
    &\mathit{nf}^{old}_{1...N^{old}}: \text{old note nullifier.}\\
    &cm^{new}_{1...N^{new}}: \text{new note commitment.}\\
    &V^{old}_{pub,color}: \text{old public value of coin with color.}\\
    &V^{new}_{pub,color}: \text{new public value of coin with color.}\\
    &block_n: \text{current block sequence number.}\\
    &h_{sig}: \text{signature.}\\
    &h_{1...N^{old}}: \text{spending signature for old note.}
\end{align*}

The merkle tree comprises both note commitments and nullifiers, where rt is the root. 

\subsubsection{Note}

A note is the basic currency unit in the system. Essential properties of a new note (output note) are summarized as follow. Note that an old note (input note) also has the same properties.
\begin{align*}
    n^{new}_i=&(a^{new}_{sk,i},T^{new}_i,C^{new}_{i,1},V^{new}_{i,1},C^{new}_{i,2},V^{new}_{i,2}, \\
    &bt^{new}_i, \rho^{new}_i,\gamma^{new}_i,h_{sig},cm^{new}_i) \\
    &\text{where new note}\\
    &a^{new}_{sk,i}: \text{spending key.} \\
    &T^{new}_i: \text{type of note\footnotemark.} \\
    &C^{new}_{i,1}: \text{color of primary coin.}\\
    &V^{new}_{i,1}: \text{value of primary coin.}\\
    &C^{new}_{i,2}: \text{color of debt coin.}\\
    &V^{new}_{i,2}: \text{value of debt coin.}\\
    &bt^{new}_i: \text{block sequence number threshold.} \\
    &\rho^{new}_i: \text{use to compute nullifier.} \\
    &\gamma^{new}_i: \text{trapdoor.}\\
    &h_{sig}: \text{unique for a pair of matching notes.}\\
    &cm^{new}_i: \text{commitment.}\\
\end{align*}
\footnotetext{0=regular note; 1=sibling note.}

For simplying discussion, it is assumed that each transacion has two input notes and two output notes. The design can be extended to support scenarios that have more than two notes. A note can be a dummy note. The asset type of dummy note is zero (color value is zero). 


\subsubsection{Witness}

Only the prover knows witnesses. He or she uses it to generate a crypto proof for the verifier.
\begin{align*}
    \omega=&(path_1,path_2,pos_1,pos_2,n^{old}_1,n^{old}_2,a^{old}_{sk,1},a^{old}_{sk,2}, \\
    &\phi, dummy^{old}_1,dummy^{old}_2,n^{new}_1,n^{new}_2, path_3,pos_3,\\
    &n^{old}_3,a^{old}_{sk,3},path_4,pos_4,nf^{old}_3) \\
    &\text{where}\\
    &path_{1...N^{old}}\ and\ pos_{1...N^{old}}:\\
    &\text{N=1 or 2. merkle tree paths of old notes.} \\
    &n^{old}_{1...N^{old}}: \text{N=1 or 2. old notes.} \\
    &a^{old}_{1...N^{old}}: \text{N=1 or 2. old spending keys.} \\
    &\phi: \text{random seed}\\
    &dummy^{old}_{1...N^{old}}: \text{old note is dummy or note.} \\
    &n^{new}_{1...N^{new}}: \text{new notes.}\\
    &path_3\ and\ pos_3:\\
    &\text{merkle tree path and position of sibling note} \\
    &\text{with one of the old notes.}\\
    &n^{old}_3: \text{sibling note with one of the old note.}\\
    &a^{old}_{sk,3}: \text{spending key of the sbling note.} \\
    &path_4\ and\ pos_4:\\
    &\text{merkle tree path and position of sibling note } \\
    &\text{nullifier.}\\
    &nf^{old}_3: \text{sibling note nullifier.}
\end{align*}

